Solving the TTC 2011 Compiler Optimization Case with GrGen.NET

The challenge of the Compiler Optimization Case is to perform local optimizations and instruction selection on the graph-based intermediate representation of a compiler. The case is designed to compare participating tools regarding their performance. We tackle this task employing the general purpose graph rewrite system GrGen.NET (www.grgen.net).

==> eptcsdata.tex <==
\providecommand{\firstpage}{42}
\providecommand{\publicationstatus}{Van Gorp, Mazanek and Rose (Eds.): \\Fifth Transformation Tool Contest (TTC 2011)\\
EPTCS 74, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.74.7}{10.4204/EPTCS.74.7}}
\pdfoutput=1

